Internal Dynamics of Multiple Populations in 28 Galactic Globular Clusters: A Wide-Field study with Gaia and the Hubble Space Telescope

We present a detailed analysis of the internal dynamics of multiple stellar populations (MPs) in 28 Galactic Globular Clusters (GCs) across a wide field of view, extending from the innermost regions to the clusters' outskirts. Using astro-photometric catalogs from ground-based observations, Gaia, and the Hubble Space Telescope (HST), we identify first- (1P) and second-population (2P) stars, and study the internal dynamics of MPs using high-precision Gaia DR3 and HST proper motions. Our results reveal that while the 1P transitions from isotropy to slight tangential anisotropy toward the outer regions, 2P stars become increasingly radially anisotropic beyond the half-light radius. We also explore the connection between the dynamics of MPs and the clusters' structural and dynamical properties, finding statistically significant differences in the anisotropy profiles of dynamically young and non-relaxed clusters, particularly beyond the 1-2 half-light radii. In these regions, 1P stars transition from isotropic to slightly tangentially anisotropic motion, while 2P stars become more radially anisotropic. In contrast, dynamically older clusters, with mixed MPs, exhibit weaker relative differences. Furthermore, clusters with orbits closer to the Galactic center exhibit larger dynamical differences between 1P and 2P stars than those with larger peri-Galactic radii. These findings are consistent with a scenario where 2P stars form in a more centrally concentrated environment, where the interaction with the Milky Way tidal field plays a crucial role in the dynamical evolution of MPs, especially of 1P.

==> table.tex <==
\rowcolors{2}{gray!25}{white}
\begin{table*}
    \caption{...}
    \centering
    \begin{tabular}{ccccccccc}
        \hline
        \hline
         & \textbf{Cluster} & \textbf{Dynanmical age} & \textbf{MPs} & \textbf{Rotation} & \textbf{Peri radius}  & $\mathbf{v_\mathrm{esc}}$ & \textbf{Origin} & \textbf{Filling factor} \\
        \hline
        \hline
        \textbf{0} & NGC0104 & young & p2conc & rot & outer & high & insitu & underfilling \\
        \textbf{1} & NGC0288 & young & mixed & norot & inner & low & accreted & filling \\
        \textbf{2} & NGC1261 & young & mixed & norot & inner & high & accreted & underfilling \\
        \textbf{3} & NGC1851 & young & p2conc & rot & inner & high & accreted & underfilling \\
        \textbf{4} & NGC1904 & unknown & p2conc & rot & inner & unknown & accreted & unknown \\
        \textbf{5} & NGC2298 & intermedold & p2conc & norot & inner & low & accreted & underfilling \\
        \textbf{6} & NGC2808 & young & p2conc & rot & inner & high & accreted & underfilling \\
        \textbf{7} & NGC3201 & young & p2conc & norot & outer & low & accreted & underfilling \\
        \textbf{8} & NGC4147 & unknown & mixed & norot & inner & unknown & accreted & unknown \\
        \textbf{9} & NGC4590 & young & mixed & norot & outer & low & accreted & underfilling \\
        \textbf{10} & NGC4833 & young & p2conc & norot & inner & low & accreted & filling \\
        \textbf{11} & NGC5053 & young & p1conc & norot & outer & low & accreted & filling \\
        \textbf{12} & NGC5904 & young & p2conc & rot & inner & high & accreted & underfilling \\
        \textbf{13} & NGC5272 & young & p2conc & rot & outer & high & accreted & underfilling \\
        \textbf{14} & NGC5927 & young & mixed & norot & outer & high & insitu & filling \\
        \textbf{15} & NGC6121 & intermedold & mixed & norot & inner & low & insitu & filling \\
        \textbf{16} & NGC6205 & young & mixed & norot & inner & high & accreted & underfilling \\
        \textbf{17} & NGC6218 & intermedold & mixed & rot & inner & low & insitu & filling \\
        \textbf{18} & NGC6254 & intermedold & p2conc & norot & inner & high & insitu & filling \\
        \textbf{19} & NGC6366 & intermedold & mixed & norot & inner & low & insitu & filling \\
        \textbf{20} & NGC6712 & unknown & p1conc & norot & inner & unknown & insitu & unknown \\
        \textbf{21} & NGC6752 & intermedold & mixed & rot & inner & high & insitu & underfilling \\
        \textbf{22} & NGC6809 & young & mixed & norot & inner & low & insitu & filling \\
        \textbf{23} & NGC6838 & intermedold & mixed & norot & outer & low & insitu & filling \\
        \textbf{24} & NGC6934 & young & mixed & norot & inner & high & insitu & underfilling \\
        \textbf{25} & NGC6981 & intermedold & p2conc & norot & inner & low & accreted & underfilling \\
        \textbf{26} & NGC7006 & unknown & p1conc & norot & inner & unknown & accreted & unknown \\
        \textbf{27} & NGC7492 & unknown & mixed & norot & inner & unknown & accreted & unknown \\
        \textbf{28} & NGC7089 & young & mixed & rot & inner & high & accreted & underfilling \\
        \hline
        \hline
    \end{tabular}
\label{tab:tab1}
\end{table*}
    
